A Bandit Approach to Maximum Inner Product Search

There has been substantial research on sub-linear time approximate algorithms for Maximum Inner Product Search (MIPS). To achieve fast query time, state-of-the-art techniques require significant preprocessing, which can be a burden when the number of subsequent queries is not sufficiently large to amortize the cost. Furthermore, existing methods do not have the ability to directly control the suboptimality of their approximate results with theoretical guarantees. In this paper, we propose the first approximate algorithm for MIPS that does not require any preprocessing, and allows users to control and bound the suboptimality of the results. We cast MIPS as a Best Arm Identification problem, and introduce a new bandit setting that can fully exploit the special structure of MIPS. Our approach outperforms state-of-the-art methods on both synthetic and real-world datasets.

==> bandit.tex <==
\section{bandit-based approach v2}

This section is based on \cite{audibert2010best}.

Assume there are $K$ arms, the budget is $n$ and $K$ probability distributions $\nu_1, \nu_2, \cdots, \nu_K$ associated respectively with arm $1$, $2$,$\cdots$, arm $K$. These distributions are in general unknown. Let $\mu_1, \cdots, \mu_K$ be the respective means of $\nu_1, \cdots, \nu_K$. 
Let $\mu^* = \mathop{max}_{k\in \{ 1, \cdots, K \}} \mu_k $.
At the end of $n$ rounds, the forecaster selects an arm, denoted by $J_n$.
The goal is to select the arm with highest mean.
 The regret of the forecaster is  
\begin{equation}
r_n = \mu^* - \mu_{J_n}
\end{equation}

Furthermore, we define the following suboptimality of arm $i$:
\begin{equation}
\Delta_{i} = \mu^* - \mu_i
\end{equation}

Let $e_n$ denote the probability of error, that is the probability that the recommendation is not the optimal one:
\begin{equation}
e_n = \mathbb{P}(J_n \neq i^*)
\end{equation} 

We have $\mathbb{E} r_n = \sum_{i \neq i^*}  \mathbb{P}(J_n = i)\Delta_i$,
consequently, 
\begin{equation}
\mathbb{E} r_n \leq e_n
\end{equation}

We introduce the notation $(i) \in \{1, \cdots, K\}$ to denote the $i$-th best arm (with ties breaks arbitrarily)

To introduce the algorithm, we need to define
\begin{equation}
\begin{split}
\overline{\log}(K) &= \frac{1}{2} + \sum_{i=2}^K \frac{1}{i} \\
n_0 &= 0 \\
n_k &= \lceil \frac{1}{\overline{\log}(K)} \frac{n-K}{K+1-k}  \rceil
\end{split}
\end{equation}

\begin{algorithm}
\caption{bandit-based best feature selectionV1}
\label{CD:bandit_best_featureV1}
\begin{algorithmic}
\STATE{\textbf{input: } $K$ arms, budget $n$  }
\STATE set $A_1 = \{ 1,\cdots, K  \}$

\FOR{$k=0,1,\cdots, K-1$}
\STATE{Select arm $i$ for $n_k - n_{k-1}$ rounds(examples) for each $i\in A_k$ }
\STATE{ Let $A_{k+1} = A_k - \mathop{arg min}_{i\in A_k}\hat{X}_{i, n_k}$ }
\ENDFOR
\STATE{\textbf{return: } the unique element of $A_K$ as $J_n$}

\end{algorithmic}
\end{algorithm}


\begin{theorem}
The probability of error $e_n$ satisifies
\begin{equation}
e_n \leq \frac{K(K-1)}{2}\exp\left(  -\frac{n-K}{\overline{\log}(K) H_2}  \right)
\end{equation}
where 
\begin{equation}
H_2 = \mathop{i\in \{ 1, \cdots, K \} i\Delta^{-2}_{(i)} }
\end{equation}
\end{theorem}


\section{bandit-based approach in context of feature selection v2}

\subsection{best-feature selection procedure}

This section is based on \cite{audibert2010best}.
We are going to discuss the procedure of getting the best feature from a set of features. This procedure will be invoked by the approximate feature selection algorithm within each iteration to select one more feature from the remaining features. 

Assume there are $K$ remaining features, the budget of examples is $n$. $1$, $2$,$\cdots$, arm $K$. Let $\mu_1, \cdots, \mu_K$ be the total losses of $K$ features when using the whole dataset. 
Let $\mu^* = \mathop{max}_{k\in \{ 1, \cdots, K \}} \mu_k $.
After using all budget, i.e. $n$ examples, the procedure selects a feature, denoted by $J_n$.
The goal is to select the feature with least total loss.
 The regret of the procedure is  
\begin{equation}
r_n =  \mu_{J_n} - \mu^*
\end{equation}

Furthermore, we define the following suboptimality of feature $i$:
\begin{equation}
\Delta_{i} =  \mu_i - \mu^*
\end{equation}

Let $e_n$ denote the probability of error, that is the probability that the recommendation is not the optimal one:
\begin{equation}
e_n = \mathbb{P}(J_n \neq i^*)
\end{equation} 

We have $\mathbb{E} r_n = \sum_{i \neq i^*}  \mathbb{P}(J_n = i)\Delta_i$,
consequently, 
\begin{equation}
\mathbb{E} r_n \leq e_n
\end{equation}

We introduce the notation $(i) \in \{1, \cdots, K\}$ to denote the $i$-th best arm (with ties breaks arbitrarily)

To introduce the algorithm, we need to define
\begin{equation}
\begin{split}
\overline{\log}(K) &= \frac{1}{2} + \sum_{i=2}^K \frac{1}{i} \\
n_0 &= 0 \\
n_k &= \lceil \frac{1}{\overline{\log}(K)} \frac{n-K}{K+1-k}  \rceil
\end{split}
\end{equation}

\begin{algorithm}
\caption{bandit-based best feature selectionV1: getBestFeature(A, n)}
\label{CD:bandit_best_featureV1}
\begin{algorithmic}
\STATE{\textbf{input: } remaining feature set $A = \{ 1,\cdots, K  \}$, budget $n$ examples  }
\STATE set $A_1 = \{ 1,\cdots, K  \}$

\FOR{$k=0,1,\cdots, K-1$}
\STATE{add $n_k - n_{k-1}$ examples for training feature $i$ for each $i\in A_k$}
\STATE{train each classifier using $n_k$ examples with feature $i$ for each $i\in A_k$ and denote its error as $\hat{X}_{i, n_k}$}
\STATE{ Let $A_{k+1} = A_k - \mathop{arg max}_{i\in A_k}\hat{X}_{i, n_k}$ }
\ENDFOR
\STATE{\textbf{return: } the unique element of $A_K$ as $J_n$}

\end{algorithmic}
\end{algorithm}


\begin{theorem}
The probability of error $e_n$ satisifies
\begin{equation}
e_n \leq \frac{K(K-1)}{2}\exp\left(  -\frac{n-K}{\overline{\log}(K) H_2}  \right)
\end{equation}
where 
\begin{equation}
H_2 = \mathop{i\in \{ 1, \cdots, K \} i\Delta^{-2}_{(i)} }
\end{equation}
\end{theorem}

\subsection{bandit-based approximate feature selection algorithm}
Assume there are in total $F$ features and the budget is $n$ examples. The algorithm that we have would be Algorithm \ref{CD:bandit}. 

\begin{algorithm}
\caption{the bandit-based algorithm}
\label{CD:bandit}
\begin{algorithmic}
\STATE{\textbf{input:} the set of $F$ features and  budget $n$ examples}
\STATE set $C = \emptyset$
\STATE set $\bar{C} = \{1,2, \cdots, F\}$

\WHILE{the size of $C$ lesss than threshold}
\STATE{invoke getBestFeature($\bar{C},n $) } and set its returned value as $j$
\STATE{$C = C\cup \{j \}$}
\STATE{$\bar{C} = \bar{C} - \{ j\}$}

\ENDWHILE
\STATE {\bfseries return} $C$
\end{algorithmic}
\end{algorithm}

\section{median elimination}

\begin{algorithm}
\caption{median elimination: getBestFeature(A, n)}
\label{CD:median_eliminationV1}
\begin{algorithmic}
\STATE{\textbf{input: } remaining feature set $A = \{ 1,\cdots, K  \}$, and $\epsilon > 0$, $\delta > 0$   }
\STATE set $S_1 = A, \epsilon_1 = \epsilon /4, \delta_1 = \delta /2, l = 1$

\WHILE{$|S_k| > 1 $}
\STATE{ sample $1/(\epsilon_k /2)^2 \log(3/ \delta_k)$ more examples to every feature $i$ in $S_k$ }
\STATE{ train a classifier corresponding to every feature and denote its empirical error as $l_{i, k}$   }
\STATE{find the median of $l_{i, k}$, denoted by $m_{k}$}
\STATE{$S_{k+1} = S_{k} - \{i: l_{i, k} > m_{k}\}  $}
\STATE{ $ \epsilon_{k+1} = \frac{3}{4}\epsilon_{k};\delta_{k+1} = \frac{1}{2}\delta_k$  }
\STATE{$k = k+1$}
\ENDWHILE

\STATE{\textbf{return: } the unique element of $S_k$ as $J_n$}

\end{algorithmic}
\end{algorithm}

\begin{theorem}
The median elimination algorithm will return an $\epsilon$-optimal feature with probablity at least $1-\delta$, and its sample complexity is 
\begin{equation}
O\left(\frac{K}{\epsilon^2}\log\left( \frac{1}{\delta} \right) \right)
\end{equation}
\end{theorem}


Let us check to see the number of examples for training at $L$-th iteration.
\begin{equation}\footnotesize
\begin{split}
&\sum_{l=1}^L \frac{1}{(\epsilon_l/2)^2}\log (3/\delta_l)\\
=& \sum_{l =1}^L\frac{4}{\epsilon_l^2}\log (3/\delta_l)\\
=& \sum_{l=1}^L \frac{4}{ \left( (\frac{3}{4})^{l-1} \epsilon/4  \right)^2  }\log (\frac{3}{\delta}2^l )\\
=& \sum_{l=1}^L \frac{4\times 16}{\epsilon^2}\left(\frac{16}{9} \right)^{l-1}\left[l\log 2 + \log(\frac{3}{\delta})  \right]\\
=& \sum_{l=1}^L \frac{64}{\epsilon^2}\left[ l(\frac{16}{9})^{l-1}\log 2 + (\frac{16}{9}^{l-1}\log(\frac{3}{\delta}))   \right]\\
=& \frac{64}{\epsilon^2}\left\{ \frac{ [ (L+1)(\frac{16}{9})^L -1 ]\frac{7}{9} - [(\frac{16}{9})^{L+1} - \frac{16}{9}]  }{(\frac{7}{9})^2}\log 2 +  \right. \\
& \left. \frac{ (\frac{16}{9})^{L+1} -\frac{16}{9}  }{\frac{7}{9}}\log(\frac{3}{\delta})   \right\}\\
=& \frac{64}{\epsilon^2} \left\{ \frac{ (L+1)(\frac{16}{9})^L\frac{7}{9} - \frac{7}{9}- (\frac{16}{9})^{L+1}+\frac{16}{9}  }{(\frac{7}{9})^2}\log 2 + \right. \\
& \left. \frac{ (\frac{16}{9})^{L+1} -\frac{16}{9}  }{\frac{7}{9}}\log(\frac{3}{\delta})   \right\}\\
=& \frac{64}{\epsilon^2} \left\{ \frac{  (L+1)(\frac{16}{9})^L \frac{7}{9}\log 2 - (\frac{16}{9})^{L+1}\log 2 + \log 2 + (\frac{16}{9})^{L+1}\frac{7}{9}\log(\frac{3}{\delta}) - \frac{7\times 16}{9\times 9}\log (\frac{3}{\delta})  }{(\frac{7}{9})^2}    \right\}\\
=& \frac{64}{\epsilon^2} \left\{ \frac{  (L+1)(\frac{16}{9})^L \frac{7}{9}\log 2 + (\frac{16}{9})^{L+1}( \frac{7}{9}\log (\frac{3}{\delta})   - \log 2) + \log 2 - \frac{7\times 16}{9\times 9}\log (\frac{3}{\delta})  }{(\frac{7}{9})^2}    \right\}\\ 
\end{split}
\end{equation}

From above equation, we could see that the number of examples at each iteration is nearly exponential with respect to the number of iterations.
In the following analysis, for simplicity, we will assume the exponential relationship between the number of examples and number of iterations.

\begin{theorem}
Assume the time complexity of classification algorithm is $g(x) = x^p$, the number examples at $l$-th iteration is $\alpha^l m$, 
and the number of active features at $l$-th iteration is $\frac{n}{2^l}$. 
In total, there is $N$ features initially. The running time of the median elimination from $L$-th iteration forward is 
\begin{equation}
Nm^p\frac{ (\frac{\alpha^p}{2})^{\log_2 N + 1} - (\frac{\alpha^p}{2})^L }{ \frac{\alpha^p}{2} - 1 }
\end{equation}  
\end{theorem}
\begin{proof}
\begin{equation}
\begin{split}
&\sum_{l= L}^{\log_2 N} \frac{N}{2^l} g(\alpha^l m)\\
=& \sum_{l= L}^{\log_2 N} \frac{N}{2^l} (\alpha^p)^l m^p\\
=& \sum_{l= L}^{\log_2 N} N \left( \frac{\alpha}{2}  \right)^l m^p\\
=& Nm^p \frac{ \left(\frac{\alpha^p}{2} \right)^{\log_2 N + 1} - \left(\frac{\alpha^p}{2} \right)^L  }{\frac{\alpha^p}{2} - 1}
\end{split}
\end{equation}
\end{proof}

On the other hand, assuming there is $M$ total examples, the running time of using the whole dataset at $L$-th iteration would be
\begin{equation}
\frac{N}{2^L} g(M) = \frac{N}{2^L} M^p
\end{equation}


\section{ideas based on MP}

Let us focus on Matching Pursuit (MP) first. Its idea is almost the same as gradient descentwith step size always being $1$ for squared loss. 
To generalize it to other loss, we consider the type of classification/regression algorithms, called \emph{generalied linear model}. 
The generalized linear model can be characterized by $L(\beta) =\frac{1}{|S|} \sum_{i\in S}l(y_i, x_i\beta) $, where $S$ is the set of examples, $y_i$ and $x_i$ is the label and feature vector of $i$-th example, $\beta$ is the real-valued coefficient vector associated with features. 
$\beta$ is initialized to be zero vector at the very begining.
For different algorithm, the loss function $l$ is different. 
For example, $l$ is logistic loss of logistic regression, hinge loss for support vector machine and so on. Note that $l$ is squared loss for MP.

At each iteration of gradient descent, we are looking for the steepest direction by checking its derivative.
Specifically, assuming $\mathbf{e}_j$ is unit vector with only $j$-th element being $1$ 
\begin{equation}
\begin{split}
&\frac{\partial L(\beta+\lambda \mathbf{e}_j) }{\partial \lambda } \\
=&\frac{1}{|S|} \sum_{i\in S} x_{ij} l'(y_i,  x_i^T(\beta+\lambda \mathbf{e}_j) )\\
\end{split}
\end{equation}
where $l'(a, b)$ is the partial derivative $\frac{\partial l(a, b)}{\partial b}$ (with respect to second argument).

Then,
\begin{equation}
\begin{split}
&\left. \frac{\partial L(\beta+\lambda \mathbf{e}_j) }{\partial \lambda }\right|_{\lambda =0} \\
=&\frac{1}{|S|} \sum_{i\in S} x_{ij} l'(y_i,  x_i^T\beta )\\
\end{split}
\end{equation}

It means that the feature selected is
\begin{equation}
\hat{j} = \mathop{arg max}_{j}\frac{1}{|S|} \left| \sum_{i\in S} x_{ij} l'(y_i,  x_i^T\beta )\right|
\end{equation}

For example, if $l$ is squared loss, i.e. $l(y_i, x_i \beta) = (y_i - x_i \beta)^2$, then 
$l'(y_i, x_i^T \beta) = -2(y_i - x_i\beta)$. Define residual $r\in \mathbb{R}^{|S|}$, such that $r_i = (y_i - x_i\beta) $.
Then $l'(y_i, x_i^T \beta) = -2r_i$.
Therefore, we have, for squared loss,
\begin{equation}
\begin{split}
\hat{j}& = \mathop{arg max}_{j}\frac{1}{|S|} \left| \sum_{i\in S} x_{ij} l'(y_i,  x_i^T\beta )\right|\\
& = \mathop{arg max}_{j}\frac{1}{|S|} \left| \sum_{i\in S} -2x_{ij}r_i\right| \\
&= \mathop{arg max}_{j}\frac{2}{|S|} \left| \langle x_{\cdot j}, r \rangle \right| \\
&= \mathop{arg max}_{j} \left| \langle x_{\cdot j}, r \rangle \right| \\
\end{split}
\end{equation}
where $x_{\cdot j}$ is the column vector comprising of $j$-th feature values from all examples in $S$. 

Note that the minium of $j$ is taken over all the remaining features, because we don't want to reconsider the previously picked features. Having said this, we could also consider all features $j$ because this is an opportunity to adjust the previous choices.


After we selected the feature $\hat{j}$, according to the gradient descent principles, we need to update $\beta$ by 
\begin{equation}
\beta_{\hat{j}} \leftarrow \beta_{\hat{j}} - \frac{1}{|S|} \sum_{i\in S} x_{i\hat{j}} l'(y_i,  x_i^T\beta )
\end{equation}
  

At each iteration, the computation that we need to do is, $\forall j$,
\begin{equation}
\frac{1}{|S|}\sum_{i\in S} x_{ij} l'(y_i,  x_i^T\beta )
\end{equation} 
This is linear with respect to the number of examples and features, which might be prohibative when the dataset is huge.

Our idea is to use subsampling to get an estimate. 
Assume $\hat{S}$ is a subsample, we are actually trying to compute $\frac{1}{|\hat{S}|} \sum_{i\in \hat{S}} x_{ij} l'(y_i,  x_i^T\beta )$. This is where bandit approach come into play. Bandit approach will provide strategy to dynamically create samples for different feature, and eliminate features that are worse. 

Taking median elimination as an example:

\begin{algorithm}
\caption{median elimination for MP: getBestFeature(A, $\beta$)}
\label{CD:median_eliminationV2}
\begin{algorithmic}
\STATE{\textbf{input: } feature set $A = \{ 1,\cdots, J  \}$, and $\epsilon > 0$, $\delta > 0$   }
\STATE set $A_1 = A, \epsilon_1 = \epsilon /4, \delta_1 = \delta /2, l = 1$
\STATE set the estimate $\hat{l}_{j, 0} = 0 \forall j\in A_1$

\WHILE{$|A_k| > 1 $}
\STATE{ sample $1/(\epsilon_k /2)^2 \log(3/ \delta_k)$ more examples to every feature $j$ in $S_k$, let the newly added example set as $S_k$ }
\STATE{ update estimates $\hat{l}_{j, k} = \frac{1}{\sum_{t= 1}^k |S_t|} (\sum_{t= 1}^{k-1} |S_t|  \hat{l}_{j, k-1}+ \sum_{i\in S_k} x_{ij} l'(y_i,  x_i^T\beta ) )$  }
\STATE{find the median of $|\hat{l}_{j, k}|$, denoted by $m_{k}$}
\STATE{$A_{k+1} = A_{k} - \{j: |\hat{l}_{j, k}| < m_{k}\}  $}
\STATE{ $ \epsilon_{k+1} = \frac{3}{4}\epsilon_{k};\delta_{k+1} = \frac{1}{2}\delta_k$  }
\STATE{$k = k+1$}
\ENDWHILE

\STATE{\textbf{return: } the unique element of $A_k$ as $J$}

\end{algorithmic}
\end{algorithm}

\begin{algorithm}
\caption{the MP-based feature selection algorithm}
\label{CD:MP_bandit}
\begin{algorithmic}
\STATE{\textbf{input:} the set of $F$ features}
\STATE set $C = \emptyset$
\STATE set $\bar{C} = \{1,2, \cdots, F\}$
\STATE set $\beta_0 = \mathbf{0}$


\WHILE{some stopping condition does NOT hold}
\STATE{invoke getBestFeature($\bar{C}$, $\beta_t$) } and set its returned value as $j$
\STATE{$C = C\cup \{j \}$}
\STATE{$\bar{C} = \bar{C} - \{ j\}$}
\STATE{$\beta_{t+1} = \mathop{arg min}_{\beta} L(\beta)$ where $\beta$ is only allowed to vary at coordiates accoding to $C$}

\STATE{$t = t+1$}

\ENDWHILE
\STATE {\bfseries return} $C$
\end{algorithmic}
\end{algorithm}


The gurantee for the suboptimality of returned feature holds in this case, as in the following theorem.


\begin{theorem}
The median elimination algorithm for MP will return an $\epsilon$-optimal feature with probablity at least $1-\delta$, and its sample complexity is
\begin{equation}
O\left(\frac{K}{\epsilon^2}\log\left( \frac{1}{\delta} \right) \right)
\end{equation}
\end{theorem}

In Algorithm \ref{CD:MP_bandit}, I outlined the framework of the feature selection based on MP. Note that the stopping condition can take various forms. For example, it could be checking the number of selected features. Or as normally used in MP, we could check the loss on the selected features to see if it is decreasing compared to last iteration. Specifically, if the loss on the selected features is NOT less than that of last iteration, then stop the feature selection program.      


\subsection{precomputing the num of iterations before switching to full data}
For the median elimination, we know exactly how many examples that we need at $t$-th iteration. Therefore, it is possible to decide the point at which we switch to full data so that we could achieve the overall minimal computational time.

Assume the number of features that is input to median elimination is $p$ and the number of examples is $n$.
Then the computational time up to (not including) $\hat{t}$-th iteration (iteration starts from 0) is 
\begin{equation}
\sum_{t = 0}^{\hat{t}-1} \frac{p}{2^{t}}\frac{1}{(\epsilon_t/2)^2}\log{3/\delta_{t}} 
\end{equation} 

If we switch to full data at $\hat{t}$-th iteration, then the computational time on full data is
\begin{equation}
\frac{p}{2^{\hat{t}}} n
\end{equation}

The overall computational time when switch at $\hat{t}$-th iteration would be
\begin{equation}
\sum_{t = 0}^{\hat{t}-1} \frac{p}{2^{t}}\frac{1}{(\epsilon_t/2)^2}\log{3/\delta_{t}} + \frac{p}{2^{\hat{t}}} n
\end{equation}

There, we should switch to full data at $T$-th iteration, where 
\begin{equation}
T = \mathop{arg min}_{0\leq\hat{t}\leq \log_2{p}} \sum_{t = 0}^{\hat{t}-1} \frac{p}{2^{t}}\frac{1}{(\epsilon_t/2)^2}\log{3/\delta_{t}} + \frac{p}{2^{\hat{t}}} n
\end{equation}

Based on the above discussion, we have the following improved median elimination for MP
\begin{algorithm}
\caption{median elimination for MP: getBestFeature(A, $\beta$)}
\label{CD:median_eliminationV2}
\begin{algorithmic}
\STATE{\textbf{input: } feature set $A = \{ 1,\cdots, J  \}$, and $\epsilon > 0$, $\delta > 0$   }
\STATE set $A_0 = A, \epsilon_0 = \epsilon /4, \delta_0 = \delta /2$
\STATE set the estimate $\hat{l}_{j, 0} = 0 \forall j\in A_1$
\STATE $K = \mathop{arg min}_{0\leq\hat{t}\leq \log_2{p}} \sum_{t = 0}^{\hat{t}-1} \frac{p}{2^{t}}\frac{1}{(\epsilon_t/2)^2}\log{3/\delta_{t}} + \frac{p}{2^{\hat{t}}} n$


\WHILE{$k<K $}
\STATE{ sample $1/(\epsilon_k /2)^2 \log(3/ \delta_k)$ more examples to every feature $j$ in $S_k$, let the newly added example set as $S_k$ }
\STATE{ update estimates $\hat{l}_{j, k} = \frac{1}{\sum_{t= 1}^k |S_t|} (\sum_{t= 1}^{k-1} |S_t|  \hat{l}_{j, k-1}+ \sum_{i\in S_k} x_{ij} l'(y_i,  x_i^T\beta ) )$  }
\STATE{find the median of $|\hat{l}_{j, k}|$, denoted by $m_{k}$}
\STATE{$A_{k+1} = A_{k} - \{j: |\hat{l}_{j, k}| < m_{k}\}  $}
\STATE{ $ \epsilon_{k+1} = \frac{3}{4}\epsilon_{k};\delta_{k+1} = \frac{1}{2}\delta_k$  }
\STATE{$k = k+1$}
\ENDWHILE

\STATE{compute $\hat{l}_{i,k} = \frac{1}{|S|}\sum_{i\in S} x_{ij} l'(y_i,  x_i^T\beta )$ where set $S$ is the whole dataset}

\STATE{\textbf{return: } the element from $A_k$ with the highest $|\hat{l}_{i,k}|$  as $J$}

\end{algorithmic}
\end{algorithm}


\section{across-iteration analysis}
Assume the simple case. Loss is squared loss, number of examples is equal to number of features. The features are orthogonal, i.e. when the data matrix is identity. The least square problem becomes
\begin{equation}
\mathop{min}_{\beta} \|Y - X\beta \|^2 = \mathop{min}_{\beta} \|Y-\beta  \|^2
\end{equation}

Let $A$ be the set of chosen features. The loss $L(A)$ is computable in closed form: we set $\beta_i= Y_i$ for $i$ in A and zero elsewhere, which results in:
\begin{equation}
L(A) = \|Y_{\bar{A}} \|^2
\end{equation}
where $\bar{A}$ is the complement of the set $A$.

The function greedy(A) is: sort the entries of $Y$ that are not in $A$ in descending order by magnitude and pick the first element.

\textbf{Question:}

\textbf{(1)}:
Is the following conjecture true?
conjecture: assume $A$ is the set of features that are selected by bandit-based algorithm and $A'$ is the set of features that are selected by greedy feature selection algorithm.
If $L(A) - L(A')< \epsilon$, we can get 
\begin{equation}
L(A\cup \{x\}) - L(A'\cup \{x'\}) <\epsilon
\end{equation}
where $x$ is greedy(A) and $x'$ is greedy(A').

Claim: This conjecture is true.
\begin{proof}
It's easy to know that
\begin{equation}
\begin{split}
L(A\cup\{x\}) &= L(A) - Y_{x}^2\\
L(A'\cup \{ x'\}) &= L(A') - Y_{x'}^2
\end{split}
\end{equation}

Since greedy feature selection will also choose the best features, i.e. the features with largest $Y_i$.
Therefore, $Y_{x'} < Y{x}$. We have
\begin{equation} \label{Eq:conjecture}
\begin{split}
L(A) - L(A') &< \epsilon\\
L(A\cup\{x\}) + Y_{x}^2 - L(A'\cup \{ x'\}) - Y_{x'}^2 &< \epsilon\\
L(A\cup\{x\}) - L(A'\cup \{ x'\}) &< \epsilon + Y_{x'}^2 - Y_{x}^2\\
L(A\cup\{x\}) - L(A'\cup \{ x'\}) &< \epsilon
\end{split}
\end{equation}
\end{proof}

\textbf{(2)}: If yes, can we allow a small amount of correlation between features? (as opposed to them being exactly orthogonal)

\textbf{(3)}: As features become very correlated, does the conjecture fail?

Claim: For the above two questions, the conjecture still holds, because the correlated features don't really matter here.

\begin{proof}
Assume all the orthogonal features are duplicated. It means that $X = [I, I]$, where $I$ is identity matrix.

One key insight is: given the set $A$ of chosen features, greedy(A) will never choose any feature that is correlated to those in $A$, because adding a correlated feature will not change the loss, i.e. loss remains the same. 
Based on this insight and inductive argument, the set $A$ of any iteration for both bandit-based algorithm and greedy feature selection will contain only uncorrelated features.   
Since greedy($A$) will never choose correlated feature, we only need to consider uncorrelated feature. To prove the conjecture, the same argument for question (1) can be applied.

Note that here we duplicate all the orthogonal features, which is the case of highly correlated features.
\end{proof}

Another more realistic case is: the bandit-based algorithm should use greedy($A$, $\epsilon$) that will return a feature whose loss is $\epsilon$-close to best feature that is not in $A$.

Therefore, we want to investigate the conjecture still holds in this case:

Assume $A$ is the set of features that are selected by bandit-based algorithm and $A'$ is the set of features that are selected by greedy feature selection algorithm.
If $L(A) - L(A')< \epsilon$, we can get
\begin{equation}
L(A\cup \{x\}) - L(A'\cup \{x'\}) <\epsilon
\end{equation}
where $x$ is greedy(A, $\epsilon$) and $x'$ is greedy(A').

Intuitively speaking, the above conjecture may not hold. This is because bandit-based algorithm may pick a feature that is worse than the one picked by greedy the next step, i.e. it could happen that $Y_{x} < Y_{x'}$ in Eq.(\ref{Eq:conjecture}).

To further undertand it, I have run some simulation for both $l_1$ loss (see Fig. \ref{error_l1}) and $l_2$ loss (see Fig. \ref{Fig:error_l2}).
I generate a list of values for $Y = [1, 1.2, 1.4, 1.7, 2.3, 2.6, 2.8, 2.9, 3.1, 3.3, 3.4, 3.6,\\ 4.1, 4.2, 4.3, 4.7, 4.9, 5.1, 5.3, 5.5, 5.9]$. At the i-th iteration, the total error deviation is $L(A) - L(A')$ and the averaged error deviation is $(L(A) - L(A'))/i$. The averaged error deviation doesn't really make much sense at this moment. Please focus on the total error deviation. The figure is obtained by averaged over 100 runs. 
It is clear to see that the total error deviation for $l_1$ loss is bounded by $\epsilon$.  

\section{across-iteration analysis V1}
At some iteratin, assume the set of selected features is $A$. Then, $\beta_{A} = \mathop{arg min}\|Y-X_A \beta  \|^2$. 
Note that $X = \{ x_1, x_2, \cdots, x_M \}$ where $x_j$ is the $j$-th feature.
For squared loss, it is easy to see that $\beta_{A} = (X_A^T X_A)^{-1} X_A^TY$ 

We assume that 
\begin{equation}
x_i^Tx_j = \left\{ {\begin{array}{ll} 
      \mu &\text{, if $i\neq j$}\\
       0 &\text{, if $i=j$}
   \end{array}}  \right.
\end{equation}
where $\mu$ is very small (close to zero).


The selected feature is
\begin{equation}
\begin{split}
J &= \mathop{arg max}_{j} \left| x_j^T Y - x_j^TX_A\beta_A  \right|\\
&= \mathop{arg max}_j  \left| x_j^T Y - x_j^TX_A(X_A^TX_A)^{-1}X_A^TY  \right|\\
&= \mathop{arg max}_j \left| x_j^T\left[Y-X_A(X_A^TX_A)^{-1}X_A^T Y \right]   \right|
\end{split}
\end{equation}

The loss of the set of selected features is
\begin{equation} \small
\begin{split}
&\|Y - X_{A\cup\{J\}}\beta_{A\cup\{J \}} \|^2\\
=& \|Y - X_{A\cup\{J \}}( X_{A\cup\{J \}}^T X_{A\cup\{J \}} )^{-1} X_{A\cup\{J \}}^TY   \|^2  \\
\approx & \|Y - [X_A, X_J]\left[  {\begin{array}{cc}   
      (X_A^TX_A)^{-1} & 0\\
       0 &   (x_J^Tx_J)^{-1}
 \end{array} } \right] \left[ { \begin{array}{c} X_A^T\\ x_J^T   \end{array} }  \right]
\|^2\\
=& \|Y - [X_A(X_A^TX_A)^{-1}X_A^T + x_J(x_J^Tx_J)^{-1}x_J^T ]Y \|^2 \\
=& \|Y - X_A(X_A^TX_A)^{-1}X_A^TY \|^2 -2Y^Tx_Jx_J^T[ Y-X_A(X_A^TX_A)^{-1}X_A^TY ] + \|x_Jx_J^TY \| \\
=& \|Y - X_A(X_A^TX_A)^{-1}X_A^TY \|^2 -2Y^Tx_Jx_J^T[ Y-X_A(X_A^TX_A)^{-1}X_A^TY ] + Y^Tx_Jx_J^TY \|  \\
\leq & \|Y - X_A(X_A^TX_A)^{-1}X_A^TY \|^2 - 2Y^Tx_Jx_J^T(1-\lambda)Y + Y^Tx_Jx_J^TY \\
= & \|Y - X_A(X_A^TX_A)^{-1}X_A^TY \|^2 + (2\lambda -1)Y^Tx_Jx_J^T Y\\
=& \| Y - X_A\beta_A   \| + (2\lambda - 1)|x_J^TY  |^2 
\end{split}
\end{equation}


Note that the approximate equation is based on the assumption of the features. The $\leq$ sign is based on
the unverified assumptions that $X_A(X_A^TX_A)^{-1}X_A^TY \leq \lambda Y$. 

If we further assume the correlation between selected feature and target vector is upper bounded, 
i.e. $|x_J^TY|\leq \lambda'$, then we could have
\begin{equation}
\|Y - X_{A\cup\{J\}}\beta_{A\cup\{J \}} \|^2 \leq \| Y - X_A\beta_A   \| + (2\lambda - 1)\lambda'^2
\end{equation} 
i.e. 
\begin{equation}
L(A\cup\{J\}) \leq L(A) + (2\lambda - 1)\lambda'^2
\end{equation}

\section{convergence theorem w.r.t. additive approx error}
We are going to give a theorem about convergence rate of OMP with approximate $(\epsilon,\delta)$-oracle. Note that OMP is used to solve the following problem in our case:
\begin{equation}
\mathop{min}_{x\in \mathop{lin}(\mathcal{A})} f(x)
\end{equation}
where $\mathcal{A}$ is the set of feature vectors, the operator $\mathop{lin}(\cdot)$ is the linear combination and $f(\cdot)$ is the loss function. 
%Note that lots of notations here is the same with 


\begin{algorithm}
\caption{OMP}
\label{CD:OMP}
\begin{algorithmic}
\STATE{\textbf{input: } the set of feature vectors $\mathcal{A}$, $\epsilon_u, \delta_u, t_u$

\STATE set $\delta = 1-(1-\delta_u)^{1/t_u}$, $\epsilon = \frac{-(9\rho - \epsilon_u t_u )  \pm \sqrt{ (8\rho -\epsilon_u t_u)^2 - 8\rho t_u(8C + 8e_0 - 4\epsilon_u)   }}{4\rho t_u}$
\STATE set $x_0\in \mathop{arg min}_{x\in \mathcal{A}}f(x) $, and $\mathcal{S} = \{ x_0\}$ 

\WHILE{$t=0,\cdots, t_u $}
\STATE{Find $z_t = (\epsilon, \delta)\text{-ORACLE}(\nabla f(x_t))$}
\STATE{$\mathcal{S} = \mathcal{S} \cup \{ z_t \}$}
\STATE{Let $b=x_t - \frac{1}{L}\nabla f(x_t)$}
\STATE{Update $x_{t+1} = \mathop{arg min}_{z\in \mathop{lin}(\mathcal{S})} \| z-b\|_2^2 $}
\ENDWHILE

\STATE{\textbf{return: } $\mathcal{S}$ as the selected set of features}

\end{algorithmic}
\end{algorithm}


Assume an $(\epsilon,\delta)$-oracle that, with probability at least $1-\delta$, will return $\tilde{z}\in \mathcal{A}$ by taking $d$ as input, s.t. 
\begin{equation}
\langle d, \tilde{z} \rangle \leq \langle d, z\rangle + \epsilon
\end{equation}
where $z = \mathop{arg min}_{a\in \mathcal{A}} \langle d, a \rangle$ and $\epsilon \geq 0$ is the additive approximate error.
Note that $\mathcal{A}$
is the set of feature vectors.
And $\mathcal{A}$ is assumed to be symmetric, i.e. it contains all opposite features. 
By doing this, OMP is trying to minimize the inner product, rather than maximize the absolute value of inner product. 

Furthermore, assume $x^*\in \mathop{arg min}_{x\in \mathop{lin}(\mathcal{A})} f(x)$.
,which is the optimal linear combination of features that minmizes the loss function.
And $x_t$ is the linear combination of features at the $t$-th iteration.
The pseudocode of OMP is shown in Algorithm \ref{CD:OMP}.

First, let us prove 
\begin{lemma}
With probability at least $1-\delta$, the following holds
\begin{equation}
\langle \nabla f(x_t), \rho \tilde{z}_t \rangle \leq -\frac{1}{2} e_t + \epsilon \rho
\end{equation}
where $e_t= f(x_t) - f(x^*)$ and $\rho \geq \mathop{max}\{ \|x^*\|_{\mathcal{A}}, \|x_0\|_{\mathcal{A}}, \cdots, \|x_T\|_{\mathcal{A}}   \}  $. 
\end{lemma}
\begin{proof}
Note that with probability at least $1-\delta$, we have $\langle d, -\rho\tilde{z} \rangle \geq \langle d,-\rho z\rangle -\rho \epsilon$
according to the definition of $(\epsilon,\delta)$-ORACLE.

\begin{equation}
\begin{split}
&\langle \nabla f(x_t), -2\rho \tilde{z}_t \rangle \\
=& \langle \nabla f(x_t), -\rho \tilde{z}_t \rangle + \langle \nabla f(x_t), -\rho \tilde{z}_t\rangle \\
\geq & \langle \nabla f(x_t), -\rho z_t\rangle - \rho \epsilon + \langle \nabla f(x_t), -\rho z_t\rangle - \rho \epsilon\\
\geq & \langle \nabla f(x_t), x_t\rangle + \langle \nabla f(x_t), -x^*\rangle - 2\rho \epsilon\\
\geq & f(x_t)- f(x^*) - 2\epsilon \rho\\
=& e_t -2 \epsilon \rho
\end{split}
\end{equation}
\end{proof} 

Then we can go ahead to prove the main theorem.
\begin{theorem}
Let $\mathcal{A}$ be a bounded and symmetric set of features such that $\rho<\infty$. 
Then, with probability at least $(1-\delta)^t$, OMP converges for $t>0$ as
\begin{equation}
f(x_t) - f(x^*) \leq \frac{8(C+e_0)}{\epsilon t + 4} + 2\epsilon \rho
\end{equation}
where $C$ is the curvature constant and $\epsilon_0$ is the initial error, i.e. $e_0 = f(x_0) - f(x^*)$. 
\end{theorem}
\begin{proof}
According to the definition of curvature $C$,
\begin{equation}
\begin{split}
f(x_{t+1})& \leq \mathop{min}_{\gamma \in [0, 1]} f(x_t) + \gamma \langle \nabla f(x_t), \rho \tilde{z}_t\rangle + \frac{\gamma^2}{2} C \\
& \leq f(x_t) + \mathop{min}_{\gamma \in  [0, 1]} \left\{ -\frac{\gamma}{2} e_t  + \gamma \epsilon \rho + \frac{\gamma^2}{2}C \right\}\\
\end{split}
\end{equation}
Note that the first inequality holds deterministically and the second one holds with probability at least $1-\delta$.
In other words, with probability at least $1-\delta$,
\begin{equation}
e_{t+1} \leq e_t + \mathop{min}_{\gamma \in  [0, 1]} \left\{ -\frac{\gamma}{2} e_t  + \gamma \epsilon \rho + \frac{\gamma^2}{2}C \right\}
\end{equation}

Set $\gamma = \frac{4}{\epsilon t + 4} \in [0, 1]$. With probability at least
$1-\delta$, then we have
\begin{equation}
\begin{split}
e_{t+1}& \leq e_t + \mathop{min}_{\gamma \in  [0, 1]} \left\{ -\frac{\gamma}{2} e_t  + \gamma \epsilon \rho + \frac{\gamma^2}{2}C \right\}\\
&\leq e_t - \frac{2}{\epsilon t + 4} (e_t - 2\epsilon \rho) + (\frac{4}{\epsilon t+ 4})^2\frac{C}{2} 
\end{split}
\end{equation}
i.e.

with probability at least $1-\delta$, the following holds
\begin{equation}
e_{t+1} - 2\epsilon \rho \leq (1-\frac{2}{\epsilon t + 4}) ( e_t - 2\epsilon \rho ) + (\frac{4}{\epsilon \rho + 4})^2\frac{C}{2}
\end{equation}

Set $\tilde{e}_t = e_t - 2\epsilon \rho$. We are going to show by induction that $\tilde{e}_t \leq  \frac{8(C+e_0)}{\epsilon t + 4}$ with probability at leat $(1-\delta)^t$.

When $t=0$, $\tilde{e}_0 = e_0 - 2\epsilon \rho \leq 2(C+ e_0)$. 
This base case is derived using the deterministic definition of $\tilde{e}_t$. Therefore, it will hold with probability $1 = (1-\delta)^0$.

Assuming $\tilde{e}_t \leq  \frac{8(C+e_0)}{\epsilon t + 4}$ with probability at least $(1-\delta)^t$, 
then
\begin{equation}
\begin{split}
\tilde{e}_{t+1}&\leq (1-\frac{2}{\epsilon t + 4}) \tilde{e}_{t} + (\frac{4}{\epsilon \rho + 4})^2\frac{C}{2} \\
&\leq (1-\frac{2}{\epsilon t + 4}) \frac{8(C +e_0)}{\epsilon t + 4} + (\frac{4}{\epsilon \rho + 4})^2\frac{C}{2} \\
&\leq (1-\frac{2}{\epsilon t + 4}) \frac{8(C +e_0)}{\epsilon t + 4} + \frac{8C}{\epsilon t + 4}\frac{1}{\epsilon t + 4} + \frac{8 e_0}{\epsilon t + 4}\frac{1}{\epsilon t + 4}\\
&= (1-\frac{2}{\epsilon t + 4}) \frac{8(C + e_0)}{\epsilon t + 4} + \frac{8(C+e_0)}{\epsilon t + 4}\frac{1}{\epsilon t + 4} \\
&=(1-\frac{2}{\epsilon t + 4} + \frac{1}{\epsilon t + 4}  ) \frac{8(C +e_0)}{\epsilon t + 4}\\
&=(1-\frac{1}{\epsilon t + 4}  ) \frac{8(C + e_0)}{\epsilon t + 4} \\
&\leq \frac{8(C + e_0)}{\epsilon t + 4} \\
&\leq \frac{8(C + e_0)}{\epsilon (t+1) + 4}\\
\end{split}
\end{equation}
Note that the first inequality holds with probablity at leat $1-\delta$, and the second inequality holds with probability at least $(1-\delta)^t$, and all the following inequalities/equalities hold deterministically. To make sure that all the steps hold, the final probability is the product of the probabilities of the first and second inequalities, i.e. $(1-\delta)^{(t+1)}$.


Therefore, with probability at least $(1-\delta)^t$, we could have
\begin{equation}
e_t \leq \frac{8(C+ e_0)}{\epsilon t + 4} + 2\epsilon \rho
\end{equation}
\end{proof}

\subsection{computing the within-iteration parameter}
When user want to get at most $t_u$ features whose error is at most $\epsilon_u$ away from that of the best features with probability at least $1- \delta_u$, we will use these input from user to compute the $\epsilon$ and $\delta$ for oracle.

(1) For $\delta$, it is easy to compute. Let $(1-\delta)^{t_u} = 1-\delta_u $. Then, we have
$\delta = 1- (1-\delta_u)^{1/t_u}$.

(2) For $\epsilon$,
\begin{equation}
\begin{split}
& \frac{8(C+ e_0)}{\epsilon t_u + 4} + 2\epsilon \rho = \epsilon_u \\
& 8(C+ e_0) + 2\epsilon \rho (\epsilon t_u + 4) = \epsilon_u (\epsilon t_u + 4) \\
& 2\rho t \epsilon^2 + (8\rho - \epsilon_u t_u)\epsilon + 8C + 8e_0 - 4\epsilon_u = 0\\
& \epsilon = \frac{-(9\rho - \epsilon_u t_u )  \pm \sqrt{ (8\rho -\epsilon_u t_u)^2 - 8\rho t_u(8C + 8e_0 - 4\epsilon_u)   }}{4\rho t_u}
\end{split}
\end{equation}



According to Theorem \ref{TH:modified_ME_sample}, we can get the sample complexity as 
\begin{equation}
O(\frac{tn}{\epsilon}\sqrt{\log \left( \frac{1}{\epsilon'} \right)})
\end{equation}
where $\epsilon'$ is the probability of the failure for multi-armed bandit.


==> framework.tex <==
\section{Framework}
This is framework.

